Machine Learning based Efficient QT-MTT Partitioning Scheme for VVC Intra Encoders

The next-generation Versatile Video Coding (VVC) standard introduces a new Multi-Type Tree (MTT) block partitioning structure that supports Binary-Tree (BT) and Ternary-Tree (TT) splits in both vertical and horizontal directions. This new approach leads to five possible splits at each block depth and thereby improves the coding efficiency of VVC over that of the preceding High Efficiency Video Coding (HEVC) standard, which only supports Quad-Tree (QT) partitioning with a single split per block depth. However, MTT also has brought a considerable impact on encoder computational complexity. In this paper, a two-stage learning-based technique is proposed to tackle the complexity overhead of MTT in VVC intra encoders. In our scheme, the input block is first processed by a Convolutional Neural Network (CNN) to predict its spatial features through a vector of probabilities describing the partition at each 4x4 edge. Subsequently, a Decision Tree (DT) model leverages this vector of spatial features to predict the most likely splits at each block. Finally, based on this prediction, only the N most likely splits are processed by the Rate-Distortion (RD) process of the encoder. In order to train our CNN and DT models on a wide range of image contents, we also propose a public VVC frame partitioning dataset based on existing image dataset encoded with the VVC reference software encoder. Our proposal relying on the top-3 configuration reaches 46.6% complexity reduction for a negligible bitrate increase of 0.86%. A top-2 configuration enables a higher complexity reduction of 69.8% for 2.57% bitrate loss. These results emphasis a better trade-off between VTM intra coding efficiency and complexity reduction compared to the state-of-the-art solutions.

==> TCSVT_2022 2/acronyms.tex <==
% A
\newacronym{avc}{AVC}{Advanced Video Coding}
%\newacronymplural{avc}{AVC}{Advanced Video Coding}

\newacronym{ai}{AI}{All Intra}
%\newacronymplural{ai}{AI}{All Intra}

\newacronym{api}{API}{Application Programming Interface}

\newacronym{awms}{AWMS}{Adaptive Workload Management Scheme}

\newacronym{acpi}{ACPI}{Advanced Configuration and Power Interface}

\newacronym{ate}{ATE}{Absolute Time Error}

\newacronym{aom}{AOM}{Alliance for Open Media}

\newacronym{arc}{ARC}{Adaptive Rate Control}
\newacronym{ann}{ANN}{artificial neural network}
\newacronym{av1}{AV1}{AOMedia Video 1}

\newacronym{alf}{ALF}{Adaptive Loop Filter}



% B
\newacronym{bd-br}{BD-BR}{Bj\o ntegaard Delta Bit Rate}
\newacronym{bd-psnr}{BD-\acrshort{psnr}}{Bj\o ntegaard Delta \acrshort{psnr}}
\newacronym{ber}{BER}{Bit Error Rate}
\newacronym{bu}{BU}{Bottom-up}
%\newacronymplural{bu}{BU}{Bottom-up}

\newacronym{bo}{BO}{Band Offset}

\newacronym{bpr}{BPR}{Bi-Prediction Refinement}
\newacronym{bt}{BT}{Binary-Tree}
% C
\newacronym{ctu}{CTU}{Coding Tree Unit}
\newacronym{cu}{CU}{Coding Unit}
\newacronym{ctb}{CTB}{Coding Tree Block}
\newacronym{cb}{CB}{Coding Block}

\newacronym{cpb}{CPB}{Current Picture Buffer}

\newacronym{cpu}{CPU}{Central Processing Unit}

\newacronym{ct}{CT}{Coding-tree partitioning}

\newacronym{cdc}{CDC}{Constrain the Docile \glspl{ctu}}

\newacronym{cdf}{CDF}{Cumulative Distribution Function}
\newacronym{cdm}{\textsc{Cdm}}{\gls{ctu} Depth Map}

\newacronym{cabac}{CABAC}{Context-Adaptive Binary Arithmetic Coding}

\newacronym{cbf}{CBF}{Coded Block Flag}

\newacronym{ccs}{CCS}{Complexity Control Scheme}

\newacronym{ctde}{CTDE}{Coding Tree Depth Estimation}
\newacronym{ccupu}{CCUPU}{Constrained Coding Units and Prediction Units}

\newacronym{ctc}{CTC}{Common Test Conditions}

\newacronym{cnn}{CNN}{Convolutional Neural Network}
\newacronym{ccitt}{CCITT}{International Telegraph and Telephone Consultative Committee}

% D
\newacronym{dvfs}{D\textsc{vfs}}{Dynamic Voltage and Frequency Scaling}
\newacronym{fd-soi}{FD-SOI}{Fully Depleted Silicon on Insulator}
\newacronym{dpm}{DPM}{Dynamic Power Management}


\newacronym{dst}{DST}{Discrete Sine Transform}
\newacronym{dct}{DCT}{Discrete Cosine Transform}

\newacronym{dbf}{DBF}{Deblocking Filter}
\newacronym{dea}{DEA}{Dominant Edge Assent}

\newacronym{dse}{DSE}{Design Space Exploration}

\newacronym{dpcm}{DPCM}{Differential Pulse-Code Modulation}
\newacronym{det}{$\Delta$ET}{$\Delta$ Encoding Time}

\newacronym{dt}{DT}{Decision Tree}

% E
\newacronym{ec}{EC}{Entropy Coding}
\newacronym{er}{ER}{Energy Reduction}

\newacronym{eo}{EO}{Edges Offset}

% F
\newacronym{frdcost}{$L_{FRD}$}{full \gls{rd} cost}
%\newacronymplural{frdcost}{$J_{FRD}$}{full \gls{rd} cost}
\newacronym{fps}{fps}{Frames per Second}
\newacronym{fvc}{FVC}{Future Video Coding}

\newacronym{fme}{FME}{Fractional Motion Estimation}

\newacronym{fdcs}{FDCS}{Fixed Depth Complexity Scaling}
\newacronym{ffmpeg}{FFmpeg}{Fast Forward \gls{mpeg}}
\newacronym{fifo}{FIFO}{First In First Out}

% G
\newacronym{gof}{GOF}{Group of Frames}
\newacronym{gop}{GOP}{Group of Pictures}
%\newacronymplural{gof}{GOF}{Groups of Frames}
\newacronym{gpu}{GPU}{Graphics Processing Unit}


% H
\newacronym{hevc}{{HEVC}}{High Efficiency Video Coding}
%\newacronymplural{hevc}{\textsc{Hevc}}{High Efficiency Video Coding}

\newacronym{hm}{HM}{\textsc{Hevc} test Model}
%\newacronymplural{hm}{HM}{HEVC test Model}

\newacronym{hd}{HD}{High Definition}

% I
\newacronym{vceg}{VCEG}{IUT-T Video Coding Experts Group}
%\newacronymplural{vceg}{VCEG}{IUT-T Video Coding Experts Group}

\newacronym{ittcc}{ITTCC}{International Telephone and Telegraph Consultative Committee}

\newacronym{ipe}{IPE}{Intra Picture Estimation}

\newacronym{ipp}{IPP}{Intra Picture Prediction}

\newacronym{ip}{IP}{Intra prediction}

\newacronym{iot}{IoT}{Internet of Things}

%\newacronymplural{iot}{IoTs}{Internet of Things}

\newacronym{im}{IM}{Intra-mode prediction}
\newacronym{isp}{ISP}{Intra Sub-Partitions}

\newacronym{itu}{ITU}{International Telecommunication Union}
\newacronym{iso}{ISO}{International Organization for Standardization}
\newacronym{iec}{IEC}{International Electrotechnical Commission}
\newacronym{itut}{ITU-T}{International Telecommunication Union Telecommunication Standardization Sector}

% J
\newacronym{jct-vc}{JCT-VC}{Joint Collaborative Team on Video Coding}
\newacronym{jvt}{JVT}{Joint Video Team}
\newacronym{jvet}{JVET}{Joint Video Experts Team}
%\newacronymplural{jct-vc}{JCT-VC}{Joint Collaborative Team on Video Coding}
\newacronym{jem}{JEM}{Joint Exploration Model}

% K
\newacronym{kld}{KLD}{Kullback-Leibler Divergence}

% L
\newacronym{ld}{LD}{Low Delay}
\newacronym{lb}{LB}{Low Delay B}
\newacronym{lp}{LP}{Low Delay P}
\newacronym{lcrdcost}{$J_{LRD}$}{low-complexity \gls{rd} cost}
%\newacronymplural{lcrdcost}{$J_{LRD}$}{low-complexity \gls{rd} cost}
\newacronym{lut}{LUT}{Look-Up Table}

\newacronym{lcb}{LCB}{Largest coding block}
\newacronym{lf}{$F_L$}{Learning Frame}
%\newacronymplural{lf}{$F_L$}{Learning Frames}
\newacronym{lgbm}{LGBM}{LightGBM}
\newacronym{lstm}{LSTM}{Long-Short Term Memory}

\newacronym{lmcs}{LMCS}{Luma Mapping with Chroma Scaling}
\newacronym{lfnst}{LFNST}{Low-Frequency Non-Separable Transform}

% M
\newacronym{mpeg}{MPEG}{ISO/IEC Moving Picture Experts Group}
%%\newacronymplural{mpeg}{M\textsc{peg}}{ISO/IEC Moving Picture Experts Group}
\newacronym{mse}{MSE}{Mean-Squared Error}
\newacronym{mep}{M\textsc{ep}}{Minimal Energy Point}
\newacronym{mep-ctu}{M\textsc{ep}-CTU}{Minimal Energy Point of \emph{\gls{ctu} level}}
\newacronym{mep-ip}{M\textsc{ep}-IP}{Minimal Energy Point of \emph{\gls{ip} level}}
\newacronym{msse}{M\textsc{sse}}{Minimization based on Search Space Exploration}
\newacronym{mcp}{M\textsc{cp}}{Minimal Cost Point}

\newacronym{mpm}{MPM}{Most Probable Mode}
\newacronym{mi}{MI}{Mutual Information}
\newacronym{msssr}{M\textsc{sssr}}{Multiple Smart Search Space Reduction}

\newacronym{ml}{ML}{Machine Learning}
\newacronym{mv}{MV}{Motion Vector}

\newacronym{mrf}{MRF}{Markov Random Field}

\newacronym{me}{ME}{Motion Estimation}
\newacronym{mc}{MC}{Motion Compensation}
\newacronym{mcc}{MCC}{Multi-Class Classifier}

\newacronym{mctdl}{MCTDL}{Motion-Compensated Tree Depth Limitation}

\newacronym{mts}{MTS}{Multiple Transform Selection}
\newacronym{mtt}{MTT}{Multi-Type Tree}
\newacronym{mrl}{MRL}{Multiple Reference Line}
\newacronym{mos}{MOS}{Mean Opinion Score}
\newacronym{movie}{MOVIE}{MOtion-tuned Video Integrity Evaluation}

\newacronym{msssim}{MS-SSIM}{Multi-Scale Structural Similarity}

\newacronym{mvd}{MVD}{Motion Vector Differences}
\newacronym{mvp}{MVP}{Motion Vector Prediction}

\newacronym{mip}{MIP}{Matrix-Based Intra Prediction}


% N
\newacronym{ni}{NI}{National Instrument}

\newacronym{ntsc}{NTSC}{National Television System Committee}

\newacronym{nmos}{NMOS}{N-type Metal Oxide Semiconductor}
\newacronym{net}{NET}{Normalized Encoding Time}
\newacronym{niqe}{NIQE}{Natural Image Quality Evaluator}
\newacronym{nal}{NAL}{Network Abstraction Layer}

% O
\newacronym{os}{OS}{Operating System}


% % P
\newacronym{pu}{PU}{Prediction Unit}
\newacronym{pb}{PB}{Prediction Block}

\newacronym{papi}{PAPI}{Performance Application Programming Interface}

\newacronym{psnr}{P\textsc{snr}}{Peak Signal-to-Noise Ratio}
\newacronym{pmos}{PMOS}{P-type Metal Oxide Semiconductor}
%\newacronym{papi}{P\textsc{api}}{Performance Application Programming Interface}

\newacronym{pdf}{PDF}{Probability Density Function}

\newacronym{pcci}{PCCI}{Percentage of Correctly Classify Instances}

\newacronym{pid}{PID}{Proportional–Integral–Derivative}

\newacronym{pi}{PI}{Proportional–Integral}

\newacronym{pal}{PAL}{Phase Alternating Line}
\newacronym{poc}{POC}{Picture Order Count}
% Q
\newacronym{q}{Q}{Quantization}
\newacronym{q-1}{Q\textsuperscript{-1}}{Inverse Quantization}
\newacronym{qp}{QP}{Quantization Parameter}
%\newacronym{qoe}{QOE}{Quality of Experience}
%\newacronym{qt}{QT}{QuadTree}
%\newacronym{qtbt}{QTBT}{QuadTree BinaryTree}

\newacronym{qoe}{QoE}{Quality of Experience}

\newacronym{qt}{QT}{Quad-Tree}

\newacronym{qtbt}{QTBT}{Quad-Tree plus Binary-Tree}
\newacronym{qtbttt}{QTBTTT}{Quad-Tree plus Binary-Tree plus Ternary-Tree}

%\newacronym{qp}{QP}{Quantization Parameter}
% R
\newacronym{rdo}{RDO}{Rate-Distortion Optimization}
%\newacronymplural{rdo}{RDO}{Rate-Distortion Optimization}
\newacronym{rapl}{R\textsc{apl}}{Running Average Power Limit}

\newacronym{rap}{RAP}{Random Access Point}

\newacronym{rdoq}{RDOQ}{Rate-Distortion Optimization Quantization}
%\newacronymplural{rdoq}{RDOQ}{Rate-Distortion Optimisation Quantization}

\newacronym{rd}{RD}{Rate-Distortion}
%\newacronymplural{rd}{RD}{Rate-Distortion}

\newacronym{rqt}{RQT}{Residual Quad-Tree}

\newacronym{ra}{RA}{Random Access}

\newacronym{rmd}{RMD}{Rough Mode Decision}

\newacronym{rsq}{$Rsq$}{Coefficient of Determination}

\newacronym{rcdm}{\textsc{Rcdm}}{Refined \gls{ctu} Depth Map}

\newacronym{rc}{RC}{Rate-Control}

\newacronym{roc}{ROC}{Receiver Operating Characteristic}

\newacronym{rpr}{RPR}{Reference Picture Resampling}

% S
\newacronym{sad}{SAD}{Sum of Absolute Differences}


\newacronym{sao}{SAO}{Sample Adaptive Offset}
\newacronym{simd}{S\textsc{imd}}{Single Instruction Multiple Data}
\newacronym{sssr}{S\textsc{ssr}}{Smart Search Space Reduction}
\newacronym{snr}{SNR}{Signal-to-Noise Ratio}

\newacronym{satd}{SATD}{Sum of Absolute Transformed Differences}
\newacronym{si}{SI}{Spatial Information}
%\newacronymplural{si}{SI}{Spatial Information}

\newacronym{svm}{SVM}{Support Vector Machine}

\newacronym{scb}{SCB}{Smallest coding block}

\newacronym{smp}{SMP}{Symmetric Motion Partition}
\newacronym{amp}{AMP}{Asymmetric Motion Partition}

\newacronym{sr}{SR}{Search Range}

\newacronym{scc}{SCC}{Subjective-driven Complexity Control}

\newacronym{sse}{SSE}{Sum of Squared Errors}
\newacronym{ssd}{SSD}{Sum of Squared Differences}
\newacronym{ssim}{SSIM}{Structural SIMilarity}
\newacronym{srr}{SRR}{SSIM Reduced-Reference}
\newacronym{sd}{SD}{Standard Definition}

% T
\newacronym{tb}{TB}{Transform Block}
\newacronym{tu}{TU}{Transform Unit}
\newacronym{t}{T}{Transform}
\newacronym{t-1}{T\textsuperscript{-1}}{Inverse Transform}

\newacronym{ti}{TI}{Temporal Information}
%\newacronymplural{ti}{TI}{Temporal Information}

\newacronym{td}{TD}{Top-Down}
%\newacronymplural{td}{TD}{Top-Down}
\newacronym{tr}{TR}{Time Reduction}

\newacronym{tstd}{Tstd}{Time Standard Deviation}

\newacronym{tt}{TT}{Ternary-Tree}
% U
\newacronym{uhd}{UHD}{Ultra High Definition}
% V
\newacronym{vdcs}{VDCS}{Variable Depth Complexity Scaling}

\newacronym{vvc}{VVC}{Versatile Video Coding}

\newacronym{vtm}{VTM}{\gls{vvc} Test Model}

\newacronym{vr}{VR}{Virtual Reality}

\newacronym{vmaf}{VMAF}{Video Multimethod Assessment Fusion}

% W
\newacronym{weka}{WEKA}{Waikato Environment for Knowledge Analysis}


% X

% Y

% Z

% Math symbols


